Complexity results for modal logic with recursion via translations and tableaux

This paper studies the complexity of classical modal logics and of their extension with fixed-point operators, using translations to transfer results across logics. In particular, we show several complexity results for multi-agent logics via translations to and from the $\mu$-calculus and modal logic, which allow us to transfer known upper and lower bounds. We also use these translations to introduce terminating and non-terminating tableau systems for the logics we study, based on Kozen's tableau for the $\mu$-calculus and the one of Fitting and Massacci for modal logic. Finally, we describe these tableaux with $\mu$-calculus formulas, thus reducing the satisfiability of each of these logics to the satisfiability of the $\mu$-calculus, resulting in a general 2EXP upper bound for satisfiability testing.

==> complexity-observ.tex <==
% !TeX root = draft.tex


We start with a few observations about the complexity of satisfiability when we have recursive operators.

	%We can similarly alter the PDL formula of the reduction in \cite{fischer1979propositional} so that it can be described by 
	%the min-fragment of the $\mu$-calculus. 
%	It follows that validity for the min- and max-fragments of the $\mu$-calculus (on one or more action) is also \EXP-complete. To see that this lower bound transfers to 
%%	these 
%	the 
%%	corresponding 
%	fragment with one action 
%%	and without variables, 
%%	\minml\ and \maxml, 
%%	it suffices to use one extra action to represent propositional variables  
%%	(for example, variable $p_i$ can be replaced by $\diam{\al}^i\diam{\beta}\true$).
%%	The argument for the one-action, no-variable fragments is more involved 
%	we can encode a one-action formula with $k$ variables into one without any, by replacing each $\Box$ by $\Box^{k+1}$ and each $\Diamond$ by $\Diamond^{k+1}$.
%%	, and for each $1 \leq i \leq k$, $p_i$ by $\Diamond^i \Box \false$.
%	It is then not hard to see that this encoding is satisfiability-preserving.

%To the best of our knowledge, there are no complexity results for the validity of logics with both LTS constraints and recursion operators.
%However, it is not hard to express in such logics that formula $\varphi$ is common knowledge, with formula $\mx X.\varphi \land [\act]X$. Since validity for $\LG_k$ with common knowledge (and without recursive operators) and $k > 1$ is \EXP-complete \cite{Halpern1992}\footnote{Similarly to Remark \ref{remark:Halpern-and-Moses-should-have-proved-more}, \cite{Halpern1992} does not explicitly cover all these cases, but the techniques can be adjusted.}, $\LG_k^\mu$ must be $\EXP$-hard.
%
%\begin{proposition}\label{prp:EXP-hard-k2}
%	Satisfiability for $\LG_k^\mu$, where $k>1$, is \EXP-hard.
%\end{proposition} 
%
%We can write that $\varphi$ is invariantly true in every state that is reachable from the current one (or, in other words, that it is common knowledge) by using the following formula: $Inv(\varphi) := \mx X.(\varphi \land [\act] X)$.
%We can also restrict the scope of the invariance to one specific action: $Inv_\al(\varphi) := \mx X. (\varphi \land [\al] X)$.
%Then, we can use these formulae to either impose that the current LTS (or the part that we have access to)
%has serial accessibility relations --- by writing $Inv(\bigwedge_{\al \in \act}\diam{\al}\true)$ --- or to simulate a modality $[i^*]$ that is based on a transitive accessibility relation --- by using $Inv_i(\varphi)$ for $[i^*]\varphi$.
%Hence, the constraints Consistency and Positive Introspection can be simulated already in the usual $\mu$-calculus. Therefore:
%
%\begin{proposition}
%	The satisfiability problem for $\d_k^\mu$, $\kf_k^\mu$, and $\df_k^\mu$ is in \EXP.
%\end{proposition} 



==> compositionality.tex <==
%!TeX root = draft.tex

%At this point we have already given translations from transitive to general frames and from serial to general frames. 

We now discuss how the conditions for frames affect each other. 
For example, to construct a transitive frame, one can take the transitive closure of a possibly non-transitive frame. 
The resulting frame will satisfy condition $4$. 
As we see, taking the closure of a frame under condition $x$ may affect whether that frame maintains condition $y$, depending on $x$ and $y$.
In the following we observe that one can apply the frame closures in certain orders that preserve the properties one aquires with each application.

%\ac{still here; the following will be restated using the same arguments}

%It is reasonable to wonder whether the translations given above are in a way ``compositional'' and could result for instance in a translation between serial \textit{and} transitive frames to general ones. 
%Here we give a general method to create new translations, by using properties of the proofs and of the frames involved. 

Let $F = (W,R)$ be a frame, $\al \in A \subseteq \act$, and $x$ a frame restriction among $T, B, 4, 5$.
Then, $\overline{R_\al}^{x}$ is the closure of $R_\al$ under $x$, 
$\overline{R}^{x,A}$ is defined by $\overline{R}^{x,A}_\beta = \overline{R_\beta}^{x}$, if $\beta \in A$, and $\overline{R}^{x,A}_\beta = R_\beta$, otherwise.
Then, $\overline{F}^{x,A} = (W,\overline{R}^{x,A})$. We make the following observation.

%\begin{theorem}\label{thm:compositionality}
%	Let $x$ be a frame restriction among $D, T, B, 4, 5$, and $y$ a frame restriction among $T, B, 4, 5$, such that $(x,y) \neq (4,B), (5,T), (5,B)$.
%	Then, for every frame $F$ that satisfies $x$, $\overline{F}^y$ also satisfies $x$.
%	For translations $\transl{x}{k}{\varphi} \text{~and~} \transl{y}{k}{\varphi}$, where $x,y \in \{\tlogic,\dlogic,\blogic,\kf, \kv\}$, we have that if the 
%	closure over property $\textsc{x}$ is preserved by applying the closure over property $\textsc{y}$, then 
%	$\transl{x}{k}{\transl{y}{k}{\varphi}} $ is satisfiable in general frames iff $\phi$ is satisfiable in frames of the property $\mathbf{XY}$.
%\end{theorem}

%\begin{proof} The proof can be found in Appendix \ref{appendix:compositionality}
%\end{proof}

\begin{lemma}\label{lem:conditionsarepreserved}
	Let $x$ be a frame restriction among $D, T, B, 4, 5$, and $y$ a frame restriction among $T, B, 4, 5$, such that $(x,y) \neq (4,B), (5,T), (5,B)$.
	Then, for every frame $F$ that satisfies $x$, $\overline{F}^y$ also satisfies $x$.
%	
	%\begin{enumerate}
	%\itemsep0em 
	%\item Seriality is preserved through transitive,reflexive,symmetric and euclidean closure (and virse-versa).
	%%\item Transitivity is preserved though serial transformation. 
	%\item Reflexivity is preserved through transitive and symmetric closure (and virse-versa) and through euclidean. 
	%
	%%\item Transitivity is preserved through reflexive closure. 
	%\item Symmetricity is preserved thought transitive and euclidean closure. 
	%
	%\item Transitivity is preserved though euclidean closure (and virse-versa). 
	%\end{enumerate}
\end{lemma}

According to Lemma \ref{lem:conditionsarepreserved}, frame conditions are preserved as seen in Figure \ref{fig:frame_hierarchy}. 
\begin{figure}
	\begin{center}
		\begin{tikzpicture}[scale=0.65,->,>=stealth',node distance=1.6cm, 
%			auto, 
			main node/.style={circle,draw,font=\large\bfseries}]
			
			%\tikzstyle{every node}+=[inner sep=2pt]
			\node (c) { };
			\node (4) [above left of=c] {$4$};
			\node (t) [below left of=c] {$T$};
			\node (b) [below right of=c] {$B$};
			\node (5) [above right of=c] {$5$};
			\node (d) [left= 4cm of c] {$D$};
			
			\path 
			(t) edge (4)
			edge [red,dashed] (5)
			edge (b)
			edge (d)
			
%			(d) edge [red,dashed] (t) 
%			edge [red,dashed, bend right] (b)
%			edge [red,dashed] (4)
%			edge [red,dashed, bend left] (5)

			(d) edge (t) 
			edge [bend right] (b)
			edge (4)
			edge [bend left] (5)
			
			(4) 
			edge (d)
			edge (5)
			edge (t)
%			(d) edge [bend left] (5)
%			edge (4)
%			edge (t)
%			edge (b)
			(b) edge [red,dashed] (4)
			edge [red,dashed] (5)
			edge (t)
			edge [bend left] (d)
			(5) edge (4)
			edge [bend right](d)
			;
		\end{tikzpicture}
	\end{center}
	\caption{The frame property hierarchy}
	\label{fig:frame_hierarchy}
\end{figure}
%
%\begin{proof}
%	The proof follows by easy algebraic property analysis. Note that when not explicitly stated, the converse does not hold. 
%\end{proof}
%
%
In Figure \ref{fig:frame_hierarchy}, an arrow from $x$ to $y$ indicates that  property $x$ is preserved though the closure of a frame under $y$. 
Dotted red arrows indicate one-way arrows.
%Condition $D$ is also included in the figure for completenes, although the closure of a transition relation is not well-defined.
For convenience, we define $\overline{F}^D = (W,\overline{R}^D)$, where $\overline{R}^D = R \cup \{ (a,a) \in W^2 \mid \centernot{\exists} (a,b) \in R \}$.
%trasformation the arrow i spointing at. 
%Dotted red arrows indicate one-way arrows.
%lines outlining transformations that preserve frame properties only in one direction. 
%As one can see, since each pair of properties has at least on path connecting it, every possible combination of frame properties can be applied sequentially while preserving the properties themselves. It suffices to always first apply the translation for the properties in the lower level (the order between them does not matter) in order to have to compositionality result. 

\begin{remark}
	We note that, in general, not all frame conditions are preserved through all closures under another condition. For example, the accessibility relation $\{(a,b),(b,b)\}$ is euclidean, but its reflexive closure $\{(a,b),(b,b),(a,a)\}$ is not.
\end{remark}


%We observe that t
There is at least one linear ordering of the frame conditions $D, T, B, 4, 5$, such that all preceding conditions are preserved 
by
%under 
closures under the following conditions. We call such an order a closure-preserving order.
%, and w
We use the linear order $D, T, B, 4, 5$ in the rest of the paper.

%\begin{corollary}
%	The satisfiability problem for any combination of frame properties of the above over the $\mu$-Calculus is in \PSPACE.
%\end{corollary}

%
%\begin{remark}
%Note that the class of frames symmetric and transitive is \textit{almost} an equivalence class. The only exception that makes it possibly several equivalence classes is the case of worlds with no neighbors, which induce their own equivalence class. This is very similar to the case of a model where the relation being an actual equivalence class, something that will become imminent later, in the many-agent case. 
%\end{remark}

==> known.tex <==
%!TeX root = draft.tex

For logic $\LG$, the satisfiability problem for $\LG$, or $\LG$-satisfiability is the problem that asks, given a formula $\varphi$, if $\varphi$ is satisfiable. Similarly, the model checking problem for $\LG$ asks if $\varphi$ is true at a given state of a given \change{finite} model. 
%\emph{the completeness problem for $\LG$} asks if $\varphi$ is complete for $\LG$.

%The classical complexity results for \ML\ are due to
 Ladner \cite{ladnermodcomp} established the classical result of \PSPACE-completeness for the satisfiability of \klogic, \tlogic, \dlogic, \kf, \df, and \sr\ and \NP-completeness for the satisfiability of \sv.  Halpern and R\^{e}go later characterized the \NP--\PSPACE\ gap  for one-action logics by the presence or absence of Negative Introspection \cite{Halpern2007Characterizing}, resulting in Theorem \ref{thm:ladhalp}. Later, Rybakov and Shkatov \cite{RybakovShkatovBComp} proved the \PSPACE-completeness of \blogic\ and \tlogic\blogic.
 For formulas with fixed-point operators, 
 D'Agostino and Lenzi in \cite{Dagostino2013S5} show that satisfiability for single-agent logics with constraint $5$ is also \NP-complete.

\begin{theorem}[\cite{ladnermodcomp,Halpern2007Characterizing,RybakovShkatovBComp}]\label{thm:ladhalp}
	If $\LG\in \{\klogic, \tlogic, \dlogic, \blogic, \tlogic\blogic, \kf, \df, \sr\}$, then 
	%	$\LG$-satisfiability is \PSPACE-complete and $\LG+5$-satisfiability is \NP-complete. Equivalently, 
	$\LG$-satisfiability is \PSPACE-complete; and $\LG+5$-satisfiability and $(\LG+5)^\mu$-satisfiability is \NP-complete.
\end{theorem}


\begin{theorem}[\cite{Halpern1992}]\label{thm:halpKkcomp}
	If $k>1$ and $\LG$ has a combination of constraints from $D, T, 4, 5$ and no recursive operators, then 
	$\LG_k$-satisfiability is \PSPACE-complete.
\end{theorem}

\begin{remark}\label{remark:Halpern-and-Moses-should-have-proved-more}
	We note that Halpern and Moses in \cite{Halpern1992} only prove these bounds for the cases of $\klogic_k, \tlogic_k, \sr_k, \logicize{KD45}_k,$ and $\sv_k$;
	and D'Agostino and Lenzi in \cite{Dagostino2013S5} only prove the \NP-completeness of satisfiability for $\sv^\mu$. However, it is not hard to see that their respective methods also work for the rest of the logics of Theorems \ref{thm:ladhalp} and \ref{thm:halpKkcomp}.
	\qedd
\end{remark}

%The following theorems give the complexity of satisfiability for the $\mu$-calculus and its fragments.

\begin{theorem}[\cite{Kozen1983a}]\label{prp:muCalc-sat}
	The satisfiability problem for the $\mu$-calculus 
	%	and \maxml\ are \PSPACE-hard and 
	is \EXP-complete.%, respectively.
\end{theorem}

%It is known that satisfiability for the min-fragment of the $\mu$-calculus (on one or more action) is \EXP-complete. It is in \EXP\ due to Theorem \ref{prp:muCalc-sat}, 
%%as so is the satisfiability problem of the $\mu$-calculus  \cite{Kozen1983a}. Furthermore, 
%and 
%this fragment  suffices \cite{Pratt_1981} to describe the PDL formula that is constructed by the reduction used in \cite{fischer1979propositional} to prove \EXP-hardness for PDL, therefore the reduction can be adjusted to prove that the min-fragment of the $\mu$-calculus  is \EXP-complete.
%%We can similarly alter the PDL formula of the reduction in \cite{fischer1979propositional} so that it can be described by 
%%the min-fragment of the $\mu$-calculus. 
%Therefore, validity for the min- and max-fragments of the $\mu$-calculus (on one or more action) is \EXP-complete. To see that this lower bound transfers to \minml\ and \maxml, it suffices to use one extra action to represent propositional variables  
%(for example, variable $x_i$ can be replaced by $\diam{\al}^i\true$).

\begin{theorem}[\cite{emerson2001model}]\label{thm:mu-calc-MC}
	The model checking problem for the $\mu$-calculus is in $\NP \cap \coNP$.\footnote{In fact, the problem is known to be in $\UP \cap \coUP$ \cite{jurdzinski1998deciding}.}
\end{theorem}

Finally we have the following initial known results about the complexity of satisfiability, when we have recursive operators. Theorems \ref{prp:fragmantsMu} and \ref{prp:EXP-hard-k2} have already been observed in \cite{AcetoAFI20}. 

\begin{theorem}\label{prp:fragmantsMu}
	The satisfiability problem for the min- and max-fragments of the $\mu$-calculus is \EXP-complete, even 
	when $|\act| = 1$. 
%	and $P = \emptyset$.
%	on one action 
%%	and for \muhml, 
%%	and even 
%%	or
%	and 
%	without propositional variables. 
%%	or without,
%%	.
\end{theorem}

\begin{proof}[Proof sketch]
	It is known that satisfiability for the min- and max-fragments of the $\mu$-calculus (on one or more action) is \EXP-complete. It is in \EXP\ due to Theorem \ref{prp:muCalc-sat}, 
	%as so is the satisfiability problem of the $\mu$-calculus  \cite{Kozen1983a}. Furthermore, 
	and 
	these fragments  suffice \cite{Pratt_1981} to describe the PDL formula that is constructed by the reduction used in \cite{fischer1979propositional} to prove \EXP-hardness for PDL. Therefore, that reduction can be adjusted to prove that 
	satisfiability for the min- and max-fragments of the $\mu$-calculus  is \EXP-complete.
\end{proof}

It is not hard to express in logics with both frame constraints and recursion operators that formula $\varphi$ is common knowledge, with formula $\mx X.\varphi \land [\act]X$. Since validity for $\LG_k$ with common knowledge (and without recursive operators) and $k > 1$ is \EXP-complete \cite{Halpern1992}\footnote{Similarly to Remark \ref{remark:Halpern-and-Moses-should-have-proved-more}, \cite{Halpern1992} does not explicitly cover all these cases, but the techniques can be adjusted.}, $\LG_k^\mu$ 
\change{is}
%must be 
$\EXP$-hard.

\begin{proposition}\label{prp:EXP-hard-k2}
	Satisfiability for $\LG_k^\mu$, where $k>1$, is \EXP-hard.
\end{proposition} 


==> negative.tex <==
% !TeX root = draft.tex


In this section, we explain how to adapt Halpern and R\^{e}go's techniques from \cite{Halpern2007Characterizing} to prove that even with recursive operators, satisfiability for one-action logics with \NI\ remains in $\NP$.
Thus, we assume in this section 
%a logic $\LG$ without recursive operators, and 
that $|\act| = 1$.
%In the course of proving the \coNP\ upper bound for logics with \NI, Halpern and R\^{e}go describe in \cite{Halpern2007Characterizing} a construction that they attribute to Nagle and Thomason \cite{nagle_thomason_1985}, which provides a  model of a particular form for a satisfiable formula. 
%From this construction, we can extract Lemma \ref{lem:NImodels} 
%and Corollary \ref{cor:smallNImodels} 
%to follow. 
%The remaining results in this section are consequence of these.

For a logic $\LG+5$, we call a 
pointed model $(\M,s)$ 
%state $s$ in an LTS
for $\LG+5$ \emph{flat} when there is a set of states $W$, such that:
\begin{itemize}
\itemsep0em 
	\item 
%	$Reach(s) = \{s\} \cup W$;
	$\M = (\{s\} \cup W,R\cup E,V)$;
	\item 
%	the restriction of $\tran$ on $Reach(s)$ is $R \cup E$, where 
			\subitem 
	$R \subseteq \{s\} \times W$ and 
			\subitem 
	$E$ is an equivalence relation on $W$; and
	\item if $\LG$ has constraint $T$, or $R\neq \emptyset$ and $\LG$ has constraint $B$, then $s \in W$.
\end{itemize}
%Lemma \ref{lem:NImodels} informs us that 
%all states are flat
%%flat states are a normal form for states of 
%for
%logics with restriction $5$.
%Negative Introspection. 
%and it is part of the construction from \cite{Halpern2007Characterizing} (proof in the Appendix).
%
\begin{lemma}[\cite{nagle_thomason_1985,Halpern2007Characterizing}]\label{lem:NImodels}
%	In an LTS with restriction $5$,
%	every state is 
%%	bisimilar to 
%	a flat state.
	Every pointed $\LG+5$-model 
	$(\M,s)$ is bisimilar to a flat pointed $\LG+5$-model.
	%	, such that 
	%	$\M' = (\{s'\} \cup W,R,V)$ and
	%%	: $W = \{s'\} \cup W'$, 
	%	$R = R_1 \cup R_2$, where $R_1 \subseteq \{s\} \times W$ and 
	%%	if $W' \neq \emptyset$, then 
	%	$R_2$ is an equivalence relation on $W$.
	%%	, otherwise $R_2 = \emptyset$.
	%	If $\LG \in \{\tlogic,\sr\}$, then $s' \in W'$.
\end{lemma}

%\begin{proof}%[Proof of Lemma \ref{lem:NImodels}]
%%	Let 
%%%	$W'$ be the set of states of $\M$ reachable from $s$ and 
%%	$T$ be the restriction of 
%%%	the accessibility relation of $\M$ 
%%	$\tran$
%%	on $Reach(s)$. 
%%	It is easy to see that the identity relation is a bisimulation from $\M$ to $\M'$, so $(\M,s) \sim (\M',s)$; \LG
%	Let 
%	$W = \{t \in Reach(s) \mid \exists t'{\in} Reach(s).~ t' \tran t \}$.
%	Therefore $Reach(s) = W \cup \{s\}$ and if $\LG \in \{\tlogic,\sr\}$, then $s \in W$. 
%	Since restriction $5$ is in effect, $\tran$ is Euclidean. Therefore, the restriction of $\tran$ on $W$ is reflexive. This in turn means that $\tran$ is symmetric in $W$: if $t_1,t_2 \in W$ and $t_1 \tran t_2$, since $t_1 \tran t$, we also have $t_2 \tran t_1$. Finally, $\tran$ is transitive in $W$: if $t_1 \tran t_2 \tran t_3$ and $t_1,t_2,t_3 \in W$, then $t_2 \tran t_1$, so $t_1 \tran t_3$ by $5$. Therefore $\tran$ is an equivalence relation when restricted on $W$ and we are done.
%\end{proof}

The  construction from \cite{ladnermodcomp} and \cite{Halpern2007Characterizing} filters the states of 
%$Reach(s)$, where $s$ is a flat state, 
the flat model, 
resulting in a small 
%state
model 
for a formula $\varphi$. 
%Using this construction, Halpern and R\^{e}go prove Corollary \ref{cor:smallNImodels} \cite[Theorem 3.1]{Halpern2007Characterizing}; the \NP\ upper bound for $\LG+5$-satisfiability of Theorem \ref{thm:ladhalp} is a direct consequence.
We adapt the proof of this result for the case where we have recursive operators.
%, and because it is of importance for what follows.

\begin{lemma}%[\cite{Halpern2007Characterizing}]
	\label{cor:smallNImodels}
	Formula
	$\varphi$ is $\LG^\mu+5$-satisfiable 
	%	iff
	if and only if 
	it is satisfied in a flat 
	pointed $\LG^\mu+5$-model
%	state 
	of 
%	size at most 
		at most 
	$O(|\varphi|)$ 
%	in an LTS for $\LG+5$.
	 states. 
\end{lemma}
\begin{proof}
The proof can be found in Appendix \ref{appendix:proofNItablo}
\end{proof}
 
\begin{theorem}
	The complexity of the satisfiability problem for logic $\LG^\mu + 5$ is \NP-complete.
\end{theorem}

\begin{proof}
	\NP-hardness is easy to see, as  propositional logic is a special case of $\LG^\mu + 5$.
	To see that satisfiability is in \NP, given a formula $\varphi$, an algorithm can nondeterministically guess a small 
	model
%	LTS 
	with a satisfying state for $\varphi$ (by Lemma \ref{cor:smallNImodels}), and then use the nondeterministic polynomial-time algorithm for model-checking $\varphi$ on 
	that model
%	the LTS 
	(by Theorem \ref{thm:mu-calc-MC}).
\end{proof}

%\newcommand{\dtf}{$\d_2\oplus\subseteq \df$\xspace}
%\section{Lower Bounds for One Action}
%
%We now prove that the satisfiability problem for every $\LG_1^\mu$ that does not have \NI\ is \EXP-hard.
%For this, we use a logic of three actions, which we call \dtf, and is an extension of $\d_3$ on actions $1,2,3$, by the following constraints on its LTSs $\diam{W,\{1,2,3\},\tran,V}$:
%\begin{enumerate}
%	\item $\xrightarrow{3}$ is transitive; and
%	\item ${\xrightarrow{1}} \cup {\xrightarrow{2}} \subseteq {\xrightarrow{3}}$.
%\end{enumerate} 
%
%\begin{theorem}[\cite{Achilleos16}]
%	The satisfiability problem for the diamond-free fragment of \dtf is \EXP-complete.
%\end{theorem}
%
%\begin{proposition}
%	If $\LG_1^\mu$ does not have \NI, then its satisfiability problem is \EXP-hard.
%\end{proposition}
%
%\begin{proof}
%	The proof is by reduction from the satisfiability problem for \dtf.
%	For a formula $\varphi$ on actions $\{1,2,3\}$ that uses no recursive operators, we define a translation $\varphi^\Diamond$.
%	Let $p$ be a propositional variable that does not appear in $\varphi$.
%	Let $setup = \mx X. \Diamond p \land \Diamond \neg p \land \Box X$, which ensures that from every state we can transition to one where .
%\end{proof}


==> stmaryrd/INSTALL <==
THE ST MARY'S ROAD SYMBOL FONT

6 APRIL 1994

This distribution contains the St Mary's Road symbol fonts:

   INSTALL       stmary5.mf    stmary8.mf    stmaryba.mf   stmaryrd.dtx
   README        stmary6.mf    stmary9.mf    stmarych.mf   stmaryrd.mf
   stmary10.mf   stmary7.mf    stmaryaj.mf   stmaryjg.mf

To install the fonts, you should:

 * run METAFONT on the fonts, for example under Unix you say:

      mf "\mode=localfont; input stmary5;"
      mf "\mode=localfont; input stmary6;"
      mf "\mode=localfont; input stmary7;"
      mf "\mode=localfont; input stmary8;"
      mf "\mode=localfont; input stmary9;"
      mf "\mode=localfont; input stmary10;"

 * move stmary*.tfm into a TeX font metrics directory

 * move stmary*.*pk into a TeX bitmaps directory

If you want to use the St Mary's Road font in LaTeX2e, you should:

 * run LaTeX2e on stmaryrd.dtx

 * move stmaryrd.sty and Ustmry.fd into a TeX inputs directory

 * read the documentation in stmaryrd.dvi

This file should only be distributed as part of the St Mary's Road
distribution.

Copyright 1994 Alan Jeffrey


==> translations-Mu-calc.tex <==
%!TeX root = draft.tex

In the remainder of this section we will modify our translations and proof technique, in order to lift our results to 
logics with fixed-point operators.
It is not clear whether the translations of Subsection \ref{subsec:trans-ml} can be extended straightforwardly in the case of logics with recursion, by using unbounded invariance $Inv$, instead of the bounded  $Inv_d$.
%It is easy to see that the translations given above would fail in the case of 
%logics with recursion -- even if we use unbounded recursion in the translation.
%existence of recursive properties. 
%This 
%is demostrated by the following example.
%can be easy seen if we take the 
%recursive property 
%formula
\begin{example}
	Let 
$\varphi_f=$ \change{$\mn$}$ X. \Box X$, which requires all paths in the model to be finite, and thus it 
is
%can 
%never be satisfied 
not satisfiable
in reflexive frames. 
In Subsection \ref{subsec:trans-ml}, to translate formulas from reflexive models, we did not need to add the negations of subformulas as conjuncts.
In this case, such a translation would give
%It is clear that 
%Assume that $\varphi_f$ is translated as 
$$\varphi_t := \varphi_f \land Inv((\Box \varphi_f \impl \varphi_f) \land (\Box\Box \varphi_f \impl \Box\varphi_f)
%\land 
%(\Box \neg\varphi_f \impl \neg\varphi_f) \land (\Box\Box \neg\varphi_f \impl \Box\neg\varphi_f)
).
$$
%$$\varphi_t := \varphi_f \land Inv((\Box \varphi_f \impl \varphi_f) \land (\Box\Box \varphi_f \impl \Box\varphi_f)
%\land 
%(\Box \neg\varphi_f \impl \neg\varphi_f) \land (\Box\Box \neg\varphi_f \impl \Box\neg\varphi_f)
%).
%$$
 \change{Indeed, on reflexive frames,} the formulas $\Box \varphi_f \impl \varphi_f$ and $\Box\Box \varphi_f \impl \Box\varphi_f$ are valid, and therefore $\varphi_t$ is equivalent to $\varphi_f$, which is \klogic-satisfiable.
% ; and 
% $\Box \neg\varphi_f \impl \neg\varphi_f$ and $\Box\Box \neg\varphi_f \impl \Box\neg\varphi_f$ are respectively equivalent to $\Diamond\true$ and $\Box \Diamond \true$.
%Therefore, $\varphi_t$ is equivalent to $\varphi_f$, a \klogic-satisfiable formula, then the translation does not preserve satisfiability in the corresponding models.
%
%Our translation though does not imply such a condition for its models and thus our proof fails. 
This was not an issue 
in Subsection \ref{subsec:trans-ml}, as
%before as 
the finiteness of the paths in a model 
cannot be expressed without recursion.

One would then naturally wonder whether conjoining over $\subc(\varphi_f)$ in the translation
 would make a difference.
The answer is affirmative, as the tranlation 
	$$ \varphi_f \wedge Inv\Bigg(\bigwedge_{\psi \in \subc(\varphi_f) } 
%	\mathsf{ax}^T[
%	cl(\psi)
\Box\psi \impl \psi 
%/ p]
\Bigg)
$$
would then yield a formula that is not satisfiable.
However, our constructions would not work to prove that such a translation preserves satisfiability.
For example, consider $\mn X.\Box(p \impl(r \land( q \impl X)))$, whose translation is satisfied on a pointed model that satisfies at the same time $p$ and $q$.
We invite the reader to verify the details.
\end{example}

%was a property not able to be captured from simple modal properties, and thus the models that had it could not be distinguished from those that did not. 
The only case \change{where} the 
%translation is still valid 
approach that we used for the logics without recursion can be applied 
is for 
the case of seriality (condition $D$), as $Inv(\diam{\al}\true)$ directly ensures the seriality of a model.
%serial frames ( i.e. the logic $\d_{\mu}^k$).

\begin{translation}
	$$ 
	\transl{A}{D^{\mu}}{\varphi}
	= \varphi  \wedge Inv\big(\bigwedge_{\al \in A}\diam{\al} \true 
	\big).$$  
\end{translation}

\begin{theorem}\label{thm:mu_calc_serial_transl}
	Let $A\subseteq \act$ and $|\act|=k$, 
	%	$x$ be one of the frame conditions, 
	and let $\LG$ be a logic, such that 
	%	Let $\LG_k$ be a logic such that 
	$\LG(\al) = \dlogic$ when $\al \in A$, and $\klogic$ otherwise.
	Then, $\varphi$ is $\LG$-satisfiable if and only if 
	$\transl{A}{D^{\mu}}{\varphi}$ is $\klogic_k^\mu$-satisfiable.
	%For every formula $\varphi$, $\transl{A}{T^{\mu}}{\varphi}$ is satisfiable in general frames iff $\varphi$ satisfiable in reflexive frames.
\end{theorem}

 

For the cases of reflexivity and transitivity, our simple translations substitute the modal subformulas of a  formula to implicitly enforce the corresponding condition.

\begin{translation}
The operation $\transl{A}{T^{\mu}}{-}$ is defined to be such that
\begin{itemize}
	\item 
$
%\transl{T^{\mu}}{K^{\mu}}{\varphi} 
\transl{A}{T^{\mu}}{[\al]\varphi}
= \stbox{\al} \transl{A}{T^{\mu}}{\varphi} \wedge \transl{A}{T^{\mu}}{\varphi}$;
\item 
$
\transl{A}{T^{\mu}}{\diam{\al}\varphi}
= \diam{\al} \transl{A}{T^{\mu}}{\varphi} \vee \transl{A}{T^{\mu}}{\varphi}$;
\item and it commutes with all other operations.
\end{itemize}
\end{translation}

\begin{theorem}\label{thm:mu_calc_reflex_translation}
	Let $\emptyset \neq A\subseteq \act$, 
%	$x$ be one of the frame conditions, 
	and let $\LG_1, \LG_2$ be logics, such that 
	%	Let $\LG_k$ be a logic such that 
	$\LG_1(\al) = \LG_2(\al) + T$ when $\al \in A$, and $\LG_2(\al)$ otherwise, and $\LG_2(\al)$ at most includes frame condition $D$.
	Then, $\varphi$ is $\LG_1$-satisfiable if and only if 
	$\transl{A}{T^{\mu}}{\varphi}$ is $\LG_2$-satisfiable.
%For every formula $\varphi$, $\transl{A}{T^{\mu}}{\varphi}$ is satisfiable in general frames iff $\varphi$ satisfiable in reflexive frames.
\end{theorem}
\begin{proof}[Proof sketch]
	The ``only if'' \change{direction} is proven by taking the appropriate reflexive closure and showing by induction that the subformulas of $\varphi$ are preserved.
The full proof can be found in Appendix \ref{appendix:proof_mu_calc_reflex_translation}
\end{proof}


\begin{translation}
	The operation $\transl{A}{4^{\mu}}{-}$ is defined to be such that
	\begin{itemize}
		\item $\transl{A}{4^{\mu}}{[\al] \psi} = Inv([\al](\transl{A}{4^{\mu}}{\psi})$, 
		\item $\transl{A}{4^{\mu}}{\diam{\al} \psi} = Eve(\diam{\al}(\transl{A}{4^{\mu}}{\psi})$\change{,}
		
		\item $\transl{A}{4^{\mu}}-$ commutes with all other operations.
		
	\end{itemize}
\end{translation}

%\ac{oh, are talking about one agent?} 

\begin{theorem}\label{thm:mu_calc_transitive_transl}
%	For every formula $\varphi$, $\transl{A}{4^{\mu}}{\varphi}$ is satisfiable if and only if $\varphi$ is satisfiable in transitive models.
	Let $\emptyset \neq A\subseteq \act$, 
	%	$x$ be one of the frame conditions, 
	and let $\LG_1, \LG_2$ be logics, such that 
	%	Let $\LG_k$ be a logic such that 
	$\LG_1(\al) = \LG_2(\al) + 4$ when $\al \in A$, and $\LG_2(\al)$ otherwise, and $\LG_2(\al)$ at most includes frame conditions $D, T, B$.
	Then, $\varphi$ is $\LG_1$-satisfiable if and only if 
	$\transl{A}{4^{\mu}}{\varphi}$ is $\LG_2$-satisfiable.
\end{theorem}


\begin{proof}
	If $\transl{A}{4^{\mu}}{\varphi}$ is satisfied in a model $M = (W,R,V)$, let $M' = (W,R^+,V)$, where $R^+_\al$ is the transitive closure of $R_\al$, if $\al \in A$, and $R^+_\al = R_\al$, otherwise.
	It is now not hard to use induction on $\psi$ to show that for every (possibly open) subformula $\psi$ of $\varphi$, for every environment $\rho$,
	$\trueset{\transl{A}{4^{\mu}}{\psi},\rho}_\M = \trueset{\psi,\rho}_{\M'}$.
	%	
	The other direction is more straightforward.
\end{proof}

In order to produce a similar translation for symmetric frames, we needed to use a more intricate type of construction. Moreover, 
we only prove the correctness of the following translation for formulas without least-fixed-point operators.
%our proof, for now, only covers formulas that are \mn-free. For those we define: 

\begin{translation}\label{transl:mu_calc_symm}
The operation $\transl{A}{\blogic^{\mu}}{-}$ is defined 
%to be such that
as
$$\transl{A}{\blogic^{\mu}}{\varphi} = \varphi \land Inv\big(\stbox{\al} \diam{\al} p \wedge \bigwedge_{\psi \in \subc(\varphi)} (\psi \rightarrow [\al][\al](p \impl \psi))\big)\change{,}$$ \change{where $p$ is a new propositional variable, not occurring in $\varphi$.}
%$\transl{A}{\blogic^{\mu}}{\varphi} = Inv(\stbox{\al} \diam{\al} p) \wedge f_A^{{\blogic^{\mu}}}(\varphi)$, where
%\begin{itemize}%{2}
%%	\item $
%%	\transl{A}{\blogic^{\mu}}{\varphi} = Inv(\stbox{\al} \diam{\al} p) \wedge f_A^{{\blogic^{\mu}}}(\varphi)$,
%		\item $
%f_A^{{\blogic^{\mu}}}({\diam{\al}\psi})= \mx X. (\diam{\al} f_A^{{B^{\mu}}}(\psi) \wedge \stbox{\al}\stbox{\al}(p \rightarrow X))$,
%\item $
%f_A^{{\blogic^{\mu}}}({\stbox{\al}\psi}) = \mx X. (\stbox{\al} f_A^{{B^{\mu}}}(\psi) \wedge \stbox{\al}\stbox{\al} (p \rightarrow X))$,
%
%	\item $f_A^{{\blogic^{\mu}}}(\psi) = \mx X. (\psi \wedge \stbox{\al}\stbox{\al}(p \rightarrow X))$, 
%	if $\psi$ is a propositional or logical variable,
%	and
%%\item $f_A^{{\blogic^{\mu}}}(X) = \mx X. (X \wedge \stbox{\al}\stbox{\al}(p \rightarrow X))$, and 
%
%\item $f_A^{{\blogic^{\mu}}}(-)$ commutes with all other operations.
%\end{itemize}
%where 
%This translation is sound, in the sense that it is satisfiable in general frames iff $\varphi$ satisfiable in reflexive frames\footnote{See proof in Appendix \ref{appendix:alt_trans}}.
\end{translation}
%
%\begin{translation}\label{transl:mu_calc_symm}
%$$ \transl{B^{\mu}}{K^{\mu}}{\varphi} =  Inv\{\stbox{\al} \diam{\al} p\} \bigwedge \varphi [(\psi \wedge \stbox{\al}\stbox{\al}(p \rightarrow \psi))/{\psi}]$$  
%where $p$ is a propositional variable that does not occur in formula $\varphi$. 
%\end{translation}

\begin{theorem}\label{thm:mu_calc_symm_translation}
	Let $\emptyset \neq A\subseteq \act$, 
%	$x$ be one of the frame conditions, 
	and let $\LG_1, \LG_2$ be logics, such that 
	%	Let $\LG_k$ be a logic such that 
	$\LG_1(\al) = \LG_2(\al) + \blogic$ when $\al \in A$, and $\LG_2(\al)$ otherwise, and $\LG_2(\al)$ at most includes frame conditions $D,T$.
	Then, a  formula $\varphi$ that has no $\mn X$ operators is $\LG_1$-satisfiable if and only if 
	$\transl{A}{\blogic^{\mu}}{\varphi}$ is $\LG_2$-satisfiable.
%For every formula $\varphi$, $\transl{A}{T^{\mu}}{\varphi}$ is satisfiable in general frames iff $\varphi$ satisfiable in reflexive frames.
\end{theorem}
\begin{proof}
The proof can be found in Appendix \ref{appendix:proof_mu_calc_summ_translation}
\end{proof}
%The case of transitivity is more straightforward:



\begin{remark}\label{remark:finitemodelB5}
	A translation for euclidean frames and for the full syntax on symmetric frames would need different approaches.
	 D'Agostino and Lenzi show in \cite{Dagostino2013S5} that $\sv_2^\mu$ does not have a finite model property, and their result can be easily extended to any logic $\LG$ with fixed-point operators, where there are at least two distinct agents $\al,\alb$, such that $\LG(\al)$ and $\LG(\alb)$ have constraint $B$ or $5$.
	 Therefore, 
	 as our constructions for the translations to $\klogic^\mu_k$ guarantee the finite model property to the corresponding logics, they do not apply to multimodal logics with $B$ or $5$.
%	 We note that 
%	 not all modal logics with recursion have a finite model property.
%	 Specifically,
\end{remark}
%A similar translation for euclidean frames and for the full syntax on symmetric frames
%
%%relative correctness proof 
%is left as future work. We conjecture that a translation similar to 
%Translation \ref{transl:mu_calc_symm}
%%the case for symmetric frames 
%would work for this scenario.
%, and we do have a candidate solution, for which we are in the process of proving the correctness. 
%However, even though we are unable to produce any counterexample for our construction, or our proof method, we still seem to be missing a few cases for completing the proof. This final result, along with the completion of the proof for the full $\mu$-Calculus over symmetric frames would yield the final upper bound for modal logic with recursion (and characterise all such logics in \EXP). Moreover as we will see later in Section \ref{sec:multi} these specific translations provide us with a very useful \textit{small model property}, as a gereralisation Kozen's result (\ref{thm:smallKmodel}) for the full $\mu$-Calculus. Thus, not only the established translations are useful for proving the termination of the tableaux we present later on, but the ones we conjecture  to exist would also immediately imply the termination of the relative presented tableaux. 

%\begin{translation}
%
%$$ \transl{\kv^{\mu}}{\klogic^{\mu}}{\varphi} = Inv_{\psi \in Sub(\varphi)}\{ (\Diamond \psi \rightarrow \Box\Diamond p_{\psi}) \wedge  (\Diamond (p_{\psi} \wedge \psi') \rightarrow \Box \Box(p_{\psi} \rightarrow \psi')) $$ $$ \wedge (\Diamond \psi \rightarrow \Diamond (\psi \wedge p_{\psi}) )\wedge (\Diamond(p_{\psi} \wedge \psi') \rightarrow \Box(p_{\psi} \rightarrow \psi')) \}
%\bigwedge \varphi [(\diam{\al}\psi \wedge \stbox{\al}\stbox{\al}(p_{\psi} \rightarrow \psi))/{\diam{\al}\psi}]
%$$  
%where the added $p_{\psi}$ are propositional variables that do not occur in formula $\varphi$ and are as many as the subformulae of $\varphi$ (and thus polynomialy many). 
%\end{translation}
%
%\begin{theorem}
%	Let $\emptyset \neq A\subseteq \act$, 
%%	$x$ be one of the frame conditions, 
%	and let $\LG_1, \LG_2$ be logics, such that 
%	%	Let $\LG_k$ be a logic such that 
%	$\LG_1(\al) = \LG_2(\al) + B$ when $\al \in A$, and $\LG_2(\al)$ otherwise, and $\LG_2(\al)$ at most includes frame condition $\kv$.
%	Then, $\varphi$ is $\LG_1$-satisfiable if and only if 
%	$\transl{A}{B^{\mu}}{\varphi}$ is $\LG_2$-satisfiable.
%%For every formula $\varphi$, $\transl{A}{T^{\mu}}{\varphi}$ is satisfiable in general frames iff $\varphi$ satisfiable in reflexive frames.
%\end{theorem}


==> translations-ml.tex <==
%!TeX root = draft.tex

 
We start with translations that map logics 
without recursive operators to logics with fewer constraints.
As mentioned in Subsection \ref{sec:known-results}, all of the logics  $\LG\in \{\klogic, \tlogic, \dlogic, \kf, \df, \sr\}$ and $\LG+5$ with one agent have known completeness results, and the complexity of modal logic is well-studied for multi-agent modal logics as well. 
The missing cases are very few and concern the combination of frame conditions (other than $5$) as well as the multi-agent case. However we take this 
%small gap as an 
opportunity to present an 
%easy and 
intuitive introduction to our general translation method.
%that can have up to one frame condition (for only one agent, these are the logics $\dlogic,\tlogic,\blogic,\kf,\kv$) to $\klogic$. 
%
%We start with translations that map logics that can have up to one frame condition (for only one agent, these are the logics $\dlogic,\tlogic,\blogic,\kf,\kv$) to $\klogic_k^\mu$.
%
%For this case, 
In fact,
the translations that we use for logics without recursion are surprisingly straightforward.
Each frame condition that we introduced in Section \ref{sec:back} is associated with an axiom for modal logic, such that whenever a model has the condition, every substitution instance of the axiom is satisfied in all worlds of the model (see \cite{blackburn2006handbook,MLBlackburnRijkeVenema,Fagin1995ReasoningAboutKnowledge}). We give  for each frame condition $x$ and agent $\al$, the axiom $\mathsf{ax}^x_\al$: 
\begin{multicols}{3}
	\begin{description}
		\item[$\ax^D_\al$: ] $\diam{\al}\true$
		\item[$\ax^T_\al$: ] $[\al]p\impl p$
		\item[$\ax^B_\al$: ] $\diam{\al}[\al]p \impl p $
		\item[$\ax^4_\al$: ] $[\al]p \impl [\al][\al]p$
		\item[$\ax^5_\al$: ] $\diam{\al}[\al]p\impl [\al]p$
	\end{description}
\end{multicols}

For each formula $\varphi$ and $d \geq 0$, let $Inv_d(\varphi) = \bigwedge_{
%	0 \leq 
	i \leq d}[\act]^i\varphi$.
%We first introduce 
Our first translations are straightforwardly defined from the above axioms.
%We now fix a certain closure-preserving order.


%We begin by presenting translations among all logics over some frame property to the logic over general frames. I.e. we give the translation of a formula that reduces the satisfiability problem for a logic over some frame property to $\klogic^{\mu}$. For this task, it turns out that the axioms corresponding to the frame properties (see preliminaries section) induce naturally a frame translation. 
%
%For the following definition, assume a frame property $x$, and the relevant axiom $ax^x $. 



\begin{translation}[One-step Translation]\label{translation:ml}
	Let $A\subseteq \act$ and let $x$ be one of the frame conditions.
	%	, and let $\LG_1 =\klogic + x$.
	%	Let $\LG_k$ be a logic such that $\LG(\al) = \LG_1$ when $\al \in A$, and $\klogic$ otherwise.
%	Then, f
	For every formula $\varphi$, let $d=md(\varphi)$ 
%	is the modal depth of $\varphi$, 
	if $x\neq 4$, and $d=md(\varphi)|\varphi|$, if $x=4$. We define:
	%$$ \transl{\LG_k^\mu}{\klogic_k^\mu}{\varphi} = \varphi \wedge Inv\Bigg(\bigwedge_{\substack{\psi \in \sub(\varphi) \\ \al \in A}} \mathsf{ax}^x_\al[cl(\psi)/ p]\Bigg).
	%$$
	$$ \transl{A}{x}{\varphi} = \varphi \wedge Inv_d\Bigg(\bigwedge_{\substack{\psi \in \subc(\varphi) \\ \al \in A}} \ax^x_\al[
%	cl(\psi)
	\psi 
	/ p]\Bigg).
	$$
	%where $ax^x[\psi\diagup p]$ stands for the axiom for logic of frame property x, with propositional formula $p$ replaced by $\psi$. 
\end{translation}

%%% If we keep the closure, we can add the following text:
%Since we do not consider recursion in the formulas, the closure of $\psi$ in the above definition is redundant.

%\begin{theorem}
%	Let $A\subseteq \act$, $x$ be one of the frame conditions, and let $\LG_1 =\klogic + x$.
%	Let $\LG_k$ be a logic such that $\LG(\al) = \LG_1$ when $\al \in A$, and $\klogic$ otherwise.
%	Then, $\varphi$ is $\LG_k$-satisfiable if and only if $ \transl{\LG_k^\mu}{\klogic_k}{\varphi}$ is $\klogic_k$-satisfiable.
%%	$$ \transl{\LG_k^\mu}{\klogic_k^\mu}{\varphi} = \varphi \wedge Inv\Big(\bigwedge_{\psi \in Sub(\varphi)} ax^x[\psi/ p]\Big).
%%	$$
%\end{theorem}

%\ac{need to alter and rearrange a bit}

\begin{theorem}\label{thm:no-fixpoint-translations-work}
	Let $A\subseteq \act$, $x$ be one of the frame conditions, and let $\LG_1, \LG_2$ be logics without recursion operators, such that 
	%	Let $\LG_k$ be a logic such that 
	$\LG_1(\al) = \LG_2(\al) + x$ when $\al \in A$, and $\LG_2(\al)$ otherwise, and $\LG_2(\al)$ only includes frame conditions that precede $x$ in the fixed order of frame conditions.
	Then, $\varphi$ is $\LG_1$-satisfiable if and only if $ \transl{A}{x}{\varphi}$ is $\LG_2$-satisfiable.
	%	$$ \transl{\LG_k^\mu}{\klogic_k^\mu}{\varphi} = \varphi \wedge Inv\Big(\bigwedge_{\psi \in Sub(\varphi)} ax^x[\psi/ p]\Big).
	%	$$
\end{theorem}
We present here a short proof sketch of this theorem.
%, in order to demonstrate the necessary steps for establishing results like this. 
%(as there will be several similar ones in the remainder of the paper). 
The full proof of Theorem \ref{thm:no-fixpoint-translations-work} can be found in Appendix \ref{appendix:Translations}
\begin{proof}[Proof sketch]
The proof of the ``only if'' direction is straightforward, as for any agent $\al$ with frame condition $x$, $\ax_\al^x$ is valid in $\LG_1$.
%The proof consists of two parts. First we prove that given a satisfiable formula $\varphi$ on frames of condition $x$ we can construct a model the its translation. In this case this direction is trivial, as any model that satisfies the frame condition $x$ also satisfies the invariant described by the translation at all reachable states, as the translation consists of the frame conditions axiom. 
%Moreover, any modal logic formula cannot describe a model at depth more than the  constant $d$, 
%in its models, 
%and t
Thus the translation holds on any $\LG_1$-model that satisfies $\varphi$. 


The other, and more involved direction 
requires the construction of an $\LG_1$-model for $\varphi$ from an $\LG_2$-model for $\transl{A}{x}{\varphi}$.
%
%Moreover, any 
We make use of the observation that no
modal logic formula can describe a model at depth more than the  constant $d$.
%
Therefore, we use the unfolding of the $\LG_2$-model, to keep track  of the path that one takes to reach a certain state, and that path's length.
We then carefully reapply the necessary closures on the accessibility relations and we use induction on its subformulas, to prove that $\varphi$ is true in the constructed model.
%consists of demonstrating the existence of a model $\M'$ of frame property $x$, given that the translation of $\varphi$ is satisfiable in some general model $\M$. For this direction and these translations the model we produce is the closure under property $x$ of $\M$. Then we proceed to prove, by induction over open subformulas of $\varphi$, and for any context $X$, that the subformulas are preserved in the $x$-closure of $\M$. 
We do this as a separate case for each axiom.
It is worth noting that we pay special care for the case of $x=4$ to account for the fact that the translation does not allow the modal depth of the relevant subformulas to decrease with each transition during the induction; and that we needed to include the negations of subformulas of $\varphi$ in the conjunction of Translation \ref{translation:ml}, only for the case of $x=5$.
\end{proof}



%%%% putting the proof here for the moment, to be moved to an appendix later
%The case-by-case proofs of this theorem (for logics $\tlogic, \dlogic, \blogic, \kf, \kv$ are given in Appendix \ref{appendix:Translations}.

%\begin{proof}
%	Assume first that $\varphi$ is satisfied in a $\LG_k^\mu$-model $\M$ and state $w$.
%	For every subformula $\psi$ of $\varphi$, $ax^x[cl(\psi)/ p]$ is an instantiation of the axiom $ax^x$, and therefore it holds at all (reachable from $w$) states of $\M$.
%	Thus, $\M,w \models Inv\Big(\displaystyle\bigwedge_{\psi \in \sub(\varphi)} ax^x[cl(\psi)/ p]\Big)$, which yields that $\M,w \models \transl{\LG_k^\mu}{\klogic_k^\mu}{\varphi}$.
%	
%	For the other direction, assume that $\M,w\models\transl{\LG_k^\mu}{\klogic_k^\mu}{\varphi}$ 
%	for some model $\M = (W,R,V)$,	
%	and state $w$.
%%	is $\klogic_k^\mu$-satisfiable.
%	For the case where $x=D$, we can see that $\M$ has a serial frame, and thus we are done.
%%	
%	For the remaining cases, let $\M' = (W,R',V)$, where $R'$ is the closure of $R$ under the condition $x$.
%	What remains is to prove that $\M',w\models \varphi$.
%	Let $\rho(X)=\trueset{cl(X)}$ for all $X$ [for this option, boxes work well, but I don't know what to do about lfps].
%	We proceed to prove that for 
%	every environment $\rho$, such that for each $X$, $\rho(X)\subseteq \trueset{cl(X)}_\M$ [lfps would work, but boxes not so well], and 
%	every $\psi \in \sub(\varphi)$, 

%\end{proof}
%
%We now proceed to prove a set of theorems, naturally occurring from the definition of the above translations.




%\begin{remark}
%As one can see we we used the contra-positive version of the axioms for symmetric and euclidean conditions on a frame. It turns out that the original axioms $ p \rightarrow \Box \Diamond p$ for symmetricity ($\Diamond p \rightarrow \Box \Diamond p$ for euclidean)  and would not induce a correct translation. To see this consider the case of a translation defined based on this version of the axiom. A non-symetric frame satisfying the translation could satisfy some formula of the form $\Box \psi'$  in a world $s$, but not satisfy $\psi'$ in all the worlds predecessors (because at this point $s$'s predecessors are not necessarily connected to it). The traslation would still be valid though, because   $\Box \Diamond \psi'$ could be valid in $s$ though it's successors. Thus there would not be a way to add symmetric edges to this model without losing the validity of $\Box \psi'$ in $s$. See figure \ref{fig:notGoodSymetricAxiom} for such an example 
%\end{remark}
%
%\begin{figure}\label{fig:notGoodSymetricAxiom}
%\begin{center}
%\begin{tikzpicture}[scale=0.6,->,>=stealth',node distance=3cm, auto, main node/.style={draw,font=\large\bfseries}]
%
%%\tikzstyle{every node}+=[inner sep=2pt]
%\node (1) {$p,q$};
%\node (2) [right = 65] {$\Box(\neg p \vee\neg q )$};
%\node (3) [above = 30,right=180] {$p,\neg q$};
%\node (4) [below = 30,right=180]{$\neg p,q$};
%
%\path 
%	(1) edge [bend right](2)
%%	    edge [red,dashed] (5)
%%	    edge (b)
%%	    edge (d)
%%	    
%    (2) edge [red,dashed,bend right](1)
%%	    edge (5)
%%	    edge (t)
%	(2) edge (3)
%		edge (4);
%\end{tikzpicture}
%\end{center}
%\caption{An example where the alternative translation for symetricity would fail.}
%\end{figure}


%
%As we saw earlier with the transition for symmetricity, we can nest some translation functions as long as model properties are preserved. In the case of the euclidean property, we see that if the initial model is reflexive, then so will be the euclidean closure of it, as all worlds have already a reflexive edge that is of course preserved. Thus we have that: 
%
%\begin{corollary} 
%The translation $\transl{t5}{k}{\varphi} = \transl{t}{k}{\transl{k5}{k}{\varphi}}$ is satisfiable in general frames iff $\varphi$ is satisfiable in reflexive \textit{and} euclidean ones. 
%\end{corollary}
%
%Note also that the above frame property (reflexive and euclidean), induced frames that are one equivalence class. Since the addition of the transitivity property to this class does not add any extra properties (it is already an equivalence class). Therefore the same translation also works for the logic $\sv$. 


\begin{corollary}\label{cor:modalupper}
	The satisfiability problem for 
	every logic without fixed-point operators
%	$\tlogic, \dlogic, \blogic, \kf, \kv$ 
	is in \PSPACE.
\end{corollary}

%\begin{corollary}
%The satisfiability problem for 
%$\tlogic^{\mu}, \dlogic^{\mu}, \blogic^{\mu}, \kf^{\mu}, \kv^{\mu}$ 
%is in \EXP.
%\end{corollary}

